Whole Brain Vessel Graphs: A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)

Biological neural networks define the brain function and intelligence of humans and other mammals, and form ultra-large, spatial, structured graphs. Their neuronal organization is closely interconnected with the spatial organization of the brain's microvasculature, which supplies oxygen to the neurons and builds a complementary spatial graph. This vasculature (or the vessel structure) plays an important role in neuroscience; for example, the organization of (and changes to) vessel structure can represent early signs of various pathologies, e.g. Alzheimer's disease or stroke. Recently, advances in tissue clearing have enabled whole brain imaging and segmentation of the entirety of the mouse brain's vasculature. Building on these advances in imaging, we are presenting an extendable dataset of whole-brain vessel graphs based on specific imaging protocols. Specifically, we extract vascular graphs using a refined graph extraction scheme leveraging the volume rendering engine Voreen and provide them in an accessible and adaptable form through the OGB and PyTorch Geometric dataloaders. Moreover, we benchmark numerous state-of-the-art graph learning algorithms on the biologically relevant tasks of vessel prediction and vessel classification using the introduced vessel graph dataset. Our work paves a path towards advancing graph learning research into the field of neuroscience. Complementarily, the presented dataset raises challenging graph learning research questions for the machine learning community, in terms of incorporating biological priors into learning algorithms, or in scaling these algorithms to handle sparse,spatial graphs with millions of nodes and edges. All datasets and code are available for download at https://github.com/jocpae/VesselGraph .

==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/01_intro.tex <==
\section{Introduction}
\label{Introduction}



Human intelligence and brain function are defined by the cerebral biological neuronal network, the so-called \textit{connectome}. The entirety of all single neurons forms an ultra-large, spatial, hierarchical and structured graph. Imaging and reconstructing these whole-brain graphs on a single-neuron level is one of the key problems in neuroscience. Neuronal organization is closely linked to the vascular network, as vessels supply the neurons with nutrients (e.g. oxygen). Specifically, the vessel topology determines the maximum metabolic load and determines neural growth patterns \cite{ji2021brain}. Vascular organisation, particularly in regards to vessel sizes and numbers of capillary links, varies substantially between brain regions, see Supplementary Figure \ref{fig:suppl_vessel_types} and \ref{fig:vessel_regions}. Moreover, its organization and changes to its structure are early signs for the development of specific diseases, e.g. Alzheimer's disease \cite{farkas2000pathological,bennett2018tau} or even COVID-19 encephalopathy \cite{uginet2021cerebrovascular}. As an initial step towards understanding the neuronal and vascular connectome (also known as the \textit{angiome} \cite{blinder2013cortical}), reliable imaging and segmentation methods are required. To this day, whole-brain imaging and segmentation of all neurons in the brain remains elusive. On the other hand, advances in tissue clearing and deep learning have enabled imaging and segmentation of the whole murine brain vasculature down to the microcapillary level \cite{todorov2020machine, kirst2020mapping}. 

Nonetheless, a binary segmentation of the vasculature is insufficient for a full, abstract description of the vascular connectome. To enable a comprehensive hierarchical description of the spatial vessel structure and anatomy, a graph representation of the brain with detailed features is required. This work provides the first large-scale, reproducible graph dataset thereof. 

% We believe that such a graph representation will facilitate research and understanding in many fields. The correction of imperfect vascular imaging and segmentation based on such an enhanced vascular graph, will enable the simulation of blood-flow (hemodynamic modeling), the study of vessel anatomy, connectivity, collateralization/anastomosis and structural abnormalities and further the understanding of many other pathologies associated with neurovascular disorders, such as stroke and dementia. 

We believe that such a graph representation can facilitate research and understanding in many fields. The correction of imperfect vascular imaging and segmentation based on such an enhanced vascular graph, could one day enable the simulation of blood-flow (hemodynamic modeling), the study of vessel anatomy, connectivity, collateralization/anastomosis and structural abnormalities. Future studies using enhanced datasets could find our approach useful to study pathologies associated with neurovascular disorders, such as stroke and dementia, given that obstacles such as plaques would be accounted for.

Evidently, the study of such spatial graphs with millions of nodes requires its own set of methods; we believe that the recent rise of advanced machine learning methods for graphs will provide suitable approaches to efficiently and accurately permit drawing deep insight from vascular graphs. This, in turn, will foster the development of methods capable of dealing with massive, but sparsely connected circular graphs, for inference on these graphs, and inference under structural and functional prior constraints that are present in such spatial physical 3D networks. 

In this work we benchmark two exemplary and biologically relevant tasks using both traditional approaches and advanced graph learning. First, in order to improve the structure and anatomical fidelity of the extracted graphs, we benchmark vessel (link) prediction. As a second task, we benchmark vessel (node) classification into the three main classes (capillaries, arterioles/venules, and arteries/veins), which represent biologically meaningful classifications by vessel size, and whose relevance for hemodynamics has been demonstrated in stroke and oxygenation modeling \cite{schmid2021severity}. 

% mention extension to the clinics on simpler datasets ? 
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.8\textwidth]{figs/Fig2.png}
	\caption{Left: 3D imaging of the whole mouse brain vasculature \cite{todorov2020machine} and right; the corresponding rendering of our whole brain spatial vessel graphs; the edges (vessels) are rendered with the average radius feature. %OTHER OPTIONS: \url{https://hmgubox2.helmholtz-muenchen.de/index.php/s/rJfHaAXppcEkWJr}
	}
	\label{fig:3d_vessel}
\end{figure}

\subsection{Whole brain vascular imaging and segmentation}

Novel imaging methods, e.g. tissue-clearing-based methods \cite{ueda2020tissue,erturk2012three,chung2013clarity,renier2014idisco}, VesSAP \cite{todorov2020machine}, Tubemap \cite{kirst2020mapping} and the work by diGiovanna et al. \cite{di2018whole} have enabled the imaging of the full vascular structure on a whole-brain scale \cite{ji2021brain}. 

The segmentation of the resulting ultra-large and unbalanced images with thousands of pixels in each dimension (e.g. $3096 \times 4719 \times 1867$ pixels \cite{todorov2020machine}) is a challenging computer vision task which is strongly affected by technical imaging imperfections. The best-performing segmentation approaches rely on deep learning, e.g. using the U-Net architecture, and are only trained on selected, manually annotated sub-volumes of the whole brain images \cite{todorov2020machine,kirst2020mapping,ji2021brain}, leading to further imperfections in the segmentation masks. 

The process presented in our work commences with segmentations of whole-brain vessel images, for which we use publicly available data from lightsheet microscopy (VesSAP), two-photon microscopy and a synthetic blood vessel dataset. For details refer to Appendix \ref{Individual_Licenses_Data}.
In the future, we will continuously increase the dataset with whole-brain images and segmentation as they become publicly available.




\subsection{Graph learning}

Machine learning on graphs is a highly relevant research field which aims to develop efficient machine learning algorithms exploiting the unique properties of graphs, such as structure neighborhoods and the sparse representation of complex systems. Our work concerns a particularly challenging domain - spatial, structured and ultra large biological graphs. In this paper we utilize and benchmark two fundamental graph learning tasks: node classification and link prediction to study the biological properties of the vascular connectome. 


A widely recognized concept for node classification is the adaption of deep learning techniques to graphs via graph convolutional networks (GCN) \cite{kipf2016semi}, a concept which was adapted and extended for many of the algorithms that we implemented, such as such as GNNs, GCNs, and GAEs \cite{kipf2016variational,zeng2019graphsaint,hamilton2017inductive,frasca2020sign,klicpera2018predict,chiang2019cluster,kong2020flag,huang2020combining,klicpera2019directional}.            
A key approach for link prediction is a so-called \textit{labeling trick} \cite{zhang2021revisiting}, which is a concept to generate sensible training data. %It has been shown to be the major contributor for the enhanced performance of some link prediction algorithms \cite{zhang2021revisiting} such as SEAL. 
The SEAL labeling trick used in our work constructs a subgraph for two candidate nodes (enclosing subgraph) and aims to learn a functional mapping on the subgraph to predict link existence \cite{zhang2018link}.



\subsection{Our contribution}

Our main contributions are: 
\begin{enumerate}
    \item We extract a set of standardized whole-brain vessel graphs based on whole, segmented murine brain images. 
    \item We publicly release said dataset in an easily accessible and adaptable format for use in graph learning benchmarking by implementing the \textit{open graph benchmark} (OGB) \cite{hu2020open} and \textit{PyTorch Geometric} data loaders \cite{fey2019fast}.
    \item In addition to our standard vessel graph, in which bifurcation points are nodes and vessels are edges, we propose an alternative representation of the vascular connectome as a line graph (where vessels become nodes), enabling the use of a multitude of advanced \textit{node classification algorithms} for vessel property prediction. 
    \item We extensively benchmark graph algorithms for the biologically important tasks of \textbf{link prediction} and \textbf{node classification}, which can serve as baselines for further research efforts in graph learning and neuroscience. 
\end{enumerate}

The rest of the paper is organized as follows: In Section \ref{Graph_Ext}, we describe our refined graph generation process and provide implementation details for the used \textit{voreen} framework and compare to other graph generation methods. We introduce the structure of our 3D brain vessel graph and provide statistics on the different extracted graphs from different brains in Section \ref{Vessel_Graph}. We describe how we generated an alternative line graph representation in Section \ref{Line_Graph}. In Section \ref{Link_Base}, we benchmark the link prediction task and in Section \ref{Node_Base}, we benchmark the node classification task on a multitude of baseline algorithms. We conclude with a focused discussion of our contribution and outline future perspectives and topics related to dataset maintenance. 



==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/03_graph.tex <==
\section{Graph extraction from segmentations}
\label{Graph_Ext}


Our graph extraction protocol begins with a given segmented whole-brain vascular dataset. Independent of segmentation method used (deep learning or filter-based), we tested the following state-of-the-art graph extraction algorithms: 1) the TubeMap method \cite{kirst2020mapping} which uses pruning on a 27-neighborhood skeletonization after a deep learning based tube-filling algorithm, based on a modified DeepVesselNet architecture \cite{tetteh2018deepvesselnet}; 2) the metric graph reconstruction algorithm by Aanjaneya et al. \cite{aanjaneya2011metric} which reduces linear connections of a skeleton to form a more compact and topologically correct graph and 3) the \textit{Voreen} vessel graph extraction method \cite{meyer2009voreen,drees2021scalable}. We tested the graph extraction algorithms on different imaging modalities, varying brain areas, and the synthetically generated vascular trees \cite{schneider2012tissue}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figs/synthetic_overview.png}
    \caption{Extracted spatial vessel graph on a synthetic vessel volume \cite{schneider2012tissue}; the graph is extracted using the \textit{Voreen} software \cite{meyer2009voreen}; a) the original vascular segmentation rendered in rendered in grey; b) depiction of the centerlines in red for a zoomed-in section; c) the nodes with a discrete colorbar encoding their degree; d) depiction of the segmentation with the edges and a continuous colorbar encoding the radius.}
    \label{fig:my_label}
\end{figure}

After expert-level evaluation of the extracted graphs in terms of feature quality, graph robustness and pipeline parameters, and of the algorithms in terms of scalability, runtime and resource constraints, we selected \textit{Voreen} \cite{drees2021scalable} for our graph generation. For details and comparisons we refer to Supplementary section \ref{Suppl_Graph_Extraction}.

\textit{Voreen} (Volume Rendering Engine) is a general framework for multi-modal volumetric dataset visualization and analysis purposes. One key advantage of \textit{Voreen} compared to other graph generation algorithms, is that its graph extraction process is deterministic, robust and scalable. It has successfully been applied to cosmological visualization \cite{scherzinger2017interactive}, visualization of large volumetric multi-channel microscopy data \cite{brix2014visualization}, 3D visualization of the lymphatic vasculature \cite{dierkes2018three}, 3D histopathology of lymphatic malformations \cite{hagerling2017vipar} and velocity mapping of the aortic flow in mice \cite{bovenkamp2015velocity}.

Our graph extraction follows a four-stage protocol:
\begin{enumerate}
    \item Skeletonization: The binary segmentation volume is reduced to a skeleton based representation by applying a standard topological thinning algorithm by Lee et al. \cite{lee1994building}.
    \item Topology Extraction: memory efficient algorithms extract the vessel centerlines \cite{isenburg2009streaming}. \textit{Voreen} allows to store this intermediate representation in a combination with the graph. 
    \item Voxel-Branch Assignment: Computing of mapping between the so-called protograph (i.e. the initial graph) and the voxels of the binary segmentation.
    \item Feature Extraction: On basis of the protograph and the mapping, several features can be computed from the foreground segmentation.
\end{enumerate}



Multiple iterations of the four-stage protocol refine and improve the graph quality and prune small, spurious branches. The key optimization parameter for the graph structure in terms of node representation, and node statistics is the \textit{bulge size}. Expert neuroscientists determined the parameter (bulge size = 3, a parameter choice in line with previous work \cite{drees2021scalable}) by statistically comparing the resulting graphs, and visually interpreting the vascular connections in varying brain regions (compare Supplementary Figure 6). Still, known limitations of topological thinning-based methods for graph extraction exist \cite{drees2021scalable}, motivating our first baseline task, presented in Section \ref{Link_Base}. % Nonetheless, the extracted graphs do not represent a perfectly connected and closed brain vasculature due to limitations in the imaging and graph extraction 



\section{3D vessel graph dataset}
\begin{table}[h!]
    \centering
    \footnotesize
    \begin{tabular}{ p{2.5cm}||p{2.2cm}|p{2cm}|p{2cm}}
    \hline
    \hline
    \multicolumn{4}{c}{Complete Datasets} \\
    \hline \hline
    Name & Number of Nodes & Num of Edges & Node Degree \\
    \hline
    BALBc1 \cite{todorov2020machine}& 3,538,495 & 5,345,897 & 3.02 \\ % final result
    BALBc2 & 3,451,306 & 5,193,775 & 3.01 \\ % final result
    BALBc3 & 2,850,347 & 4,097,953 & 2.88 \\ % final result
    C57BL/6-1  & 3,820,133 &  5,614,677 & 2.94 \\  % final result
    C57BL/6-2  & 3,439,962 &  5,070,439 & 2.95 \\  % final
    C57BL/6-3  & 3,318,212 &  4,819,208 & 2.90  \\ % final result
    CD1-E-1 & 3,645,963 & 5,791,309 & 3.18 \\ % final result
    CD1-E-2 & 1,664,811 & 2,150,326 & 2.58 \\ % final result
    CD1-E-3 & 2,295,360 & 3,130,650 & 2.73 \\ % final result
    \hline
    C57BL/6-K18 \cite{ji2021brain} & 4,284,051 & 6,525,881 & 3.05 \\ % final
    C57BL/6-K19 & 3,948,612 & 5,999,958  & 3.04 \\ % final
    C57BL/6-K20 & 4,165,085 & 6,317,179 & 3.03 \\ % final

    \hline
    Synth. Graph 1 \cite{schneider2012tissue} & 3159& 3234 & 2.05   \\
    Synth. Graph 2 & 3349 & 3421 & 2.04  \\
    Synth. Graph 3 & 3227& 3310 & 2.05 	 \\
    Synth. Graph 4 & 3178 & 3251 & 2.05  \\
    Synth. Graph 5 & 3294 & 3376 & 2.05  \\
    \hline
    
    \end{tabular}
        \caption{Total number of edges, nodes and average node degree for the different whole brain graphs.} %Please note that a standard bifurcation node has a degree of 3.}
    \label{tab:graph_numbers_nodes_edges}
\end{table}


Our 3D vessel dataset features 17 graphs from 2 different imaging modalities as well as 5 sets of synthetic vascular graphs. We found the smaller synthetic graphs useful for prototyping since they are smaller in size and cover all three classes of vessels (arteries, arterioles and capillaries). For all real vessel graphs, the full 3D images and binary segmentations are also publicly available. An overview of the notation used throughout the following sections alongside typical values can be found in Table \ref{tab:graph_feats}. 



\subsection{Vessel graph G}
\label{Vessel_Graph}

The output of the \textit{Voreen} graph extraction pipeline represents our primary unweighted and undirected graph or \say{intuitive} vessel graph. Let this graph be denoted as $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is the set of nodes and $\mathcal{E}$ is the set of all the edges of the graph.  %In biological terms the link prediction can be interpreted as "missing vessel" prediction or "correct vessel structure" prediction. 



\paragraph{Nodes:}
From a biological perspective, each node $n\in \mathcal{V}$ in our graph either represents end points of the vessel branches or the bifurcation of vessel branches, (see Figure \ref{fig:graphs}). Bifurcation points are the points where a larger vessel branches into two or more smaller vessels (in case of an artery) or smaller vessels merge into a large vessel (in case of a vein). The number of vessels branching from a bifurcation point defines the degree of that particular node. Bifurcation points have node degree of 3 or higher. In some cases, our graphs also have vessel endpoints, which are encoded as nodes of degree 1. Further, degree 2 nodes are generated by the graph extraction in cases when vessels exhibit a large curvature. These nodes are important to preserve the vessel curvature in its graph representation. For a statistical evaluation of the node degree please see Supplementary Figure \ref{fig:bulge}.

\begin{table}[h!]
    \centering
    \footnotesize
    \begin{tabular}{ p{1.5cm}|p{2.5cm}|p{1.9cm}|p{4.5cm} }
    \hline
    \hline
    \multicolumn{4}{c}{Feature Overview} \\
    \hline
    \hline
    Name & Feature Type & Value & Description  \\
    \hline
    $x_n$ & node feature & $[178,3096]$ * & x-coordinate  \\
    $y_n$ & node feature & $[808,4719]$ * & y-coordinate  \\
    $z_n$ & node feature & $[0,1866]$ * & z-coordinate  \\
    $a_n$ & node feature & $\{0,1\}^{71}$ & Allen mouse brain atlas region  \\
    \hline
    \hline
    $\mu^{r}_{ij}$ & edge feature & $[0.5,38.65]$ & mean of minimum radii  \\
    $\sigma^{r}_{ij}$ & edge feature & $[0.0,12.49]$ & std. of minimum radii\\
    $\mu^{\bar{r}}_{ij}$ & edge feature & $[0.79,38.65]$ & mean of average radii\\
    $\sigma^{\bar{r}}_{ij}$ & edge feature & $[0.0,11.99]$ & std. of minimum radii\\
    $\mu^{R}_{ij}$ & edge feature & $[0.91,44.12]$ & mean of maximum radii   \\
    $\sigma^{R}_{ij}$ & edge feature & $[0.0,23.64]$ & std. of minimum radii\\
    \hline
    $\mu^o_{ij}$ & edge feature & $[0.04,1.99]$ & mean of roundness   \\
    $\sigma^o_{ij}$ & edge feature & $[0.0,1.0]$ & std. of roundness\\
    
    \hline
    $l_{ij}$ & edge feature & $[2,322.81]$ & vessel length\\
    $d_{ij}$ & edge feature & $[1.77,300.36]$ & shortest distance\\
    $\rho_{ij}$ & edge feature & $[0.18,27.43]$ & curvature  \\
    $\alpha_{ij}$ & edge feature & $[0.29,1587.49]$ & mean crosssection area   \\
    \hline
    $v_{ij}$ & edge feature & $[1.0,119459]$ & Volume of vessel   \\
    $nv_{ij}$  & edge feature & $[0.0,256] \cap\mathbb{N}$ & no. of voxel in vessel   \\
    
    \hline
    $\nu^1_{ij}$ & edge feature & $[1,14]\cap\mathbb{N}$ & degree of $n_i$ of edge $e_{ij}$ \\
    $\nu^2_{ij}$ & edge feature & $[1,14]\cap\mathbb{N}$ & degree of $n_j$ of edge $e_{ij}$  \\
    % hasNodeAtSampleBorder && flag if node is at volume border & TBD   \\
    % isAtSampleBorder && flag if node is at volume border & TBD   \\
    
    \hline
    \hline
    \end{tabular}
    \caption{Systematic overview of the notation of the existing node and edge features in our spatial vessel graphs. All features besides the Allen brain atlas region and the node degree are spatial and extracted using Voreen, discrete ranges are given for the \textit{Balbc1} brain (* subject to imaging resolution). }
    \label{tab:graph_feats}
\end{table}


\paragraph{Node features:}
We extract two important features for the nodes of graph $\mathcal{G}$. For each node, the key features are the physical location in the coordinate space and the anatomical location in reference to the Allen brain atlas \cite{sunkin2012allen}. For the physical location feature, we denote real valued coordinates $[x_n, y_n, z_n] \in \mathbb{R}^3 \; \forall n \in \mathcal{V}$ where $[x_n, y_n, z_n]$ is the location of node $n$ in 3D space. Further, multiple prior works have shown that regional differences in vessel geometry can be observed in different brain regions \cite{ji2021brain,hahn2021large,todorov2020machine}. This motivates us to include anatomical location features for the nodes. Hence, we register the whole segmentation volume to the Allen brain atlas. Our reference Atlas uses the ontology the Allen mouse brain atlas (CCFv3 201710). We use the average template. After appropriate downsampling of the Allen brain atlas and the images, we apply a two-step-rigid and deformable registration using \textit{elastix}. Our protocol is thus identical to the Vessap paper\cite{todorov2020machine}.  Subsequently, we assign the brain region where a particular node is located in the brain atlas as anatomical node location feature, see Supplementary Figure \ref{fig:atlas_image}. Formally, the anatomical location feature $a_n=c \; \forall n \in \mathcal{V}$ if $[x_n, y_n, z_n]\in \; A_c$, where $A_c$ is the $c$\textsuperscript{th} region of the brain atlas. The atlas includes $71$ brain regions which are hierarchically clustered from $>2000$ subregions. The anatomical location feature is embedded as a one-hot encoded vector.


\paragraph{Edges:}
Each edge $e_{ij} \in \mathcal{E}$ in our graph represents vessels or vessel segments which connect two nodes $\mathcal{V}$, see Figure \ref{fig:graphs}. These edges (vessels) determine the structure of the whole brain network and represent the core aspect of our research questions. The edges exhibit the following rich set of features, which are extracted based on the shape and topology of the given segmented images.

\paragraph{Edge features:}
We extract geometric properties for each of the edges. For that, we determine the maximum diameter inscribed circle, least square reference circle, and minimum circumscribed circle on the discretized cross-section of a vessel branch and compute their radius as $\{r^k_{ij}\}, \{\bar{r}^k_{ij}\}$ and $\{R^k_{ij}\}$ where $k=1:K$ for $K$ number of cross section of the edge $e_{ij}$, respectively. From this, we compute the mean and standard deviation of the minimum, average and maximum radius for each edge $e_{ij}$ as follows. Specifically, $\mu^r_{ij}, \sigma^r_{ij}$ denotes the mean and standard deviation of minimum radius of edge $e_{ij}$. We extend the same notation for mean and standard deviation for $\{\bar{r}^k_{ij}\}$ and $\{R^k_{ij}\}$ as $\mu^{\bar{r}}_{ij}, \sigma^{\bar{r}}_{ij}, \mu^{R}_{ij}, \mu^{R}_{ij}$ respectively. We compute the roundness of each cross section as $o^k_{ij}=\frac{r^k_{ij}}{R^k_{ij}}$. We denote the mean and standard deviation of roundness as $\mu^o_{ij}$ and $\sigma^o_{ij}$, respectively. Further, we extract the vessel length $l_{ij}$, shortest distance between two nodes of an edge $d_{ij}$, curvature $\rho_{ij}=\frac{l_{ij}}{d_{ij}}$, mean cross section are $\alpha_{ij}$. Moreover, we use the degree of the nodes $n_i$ and $n_j$ for an edge $e_{ij}$ as $\nu_i$ and $\nu_j$, respectively. The complete set of edge features can be found in Table \ref{tab:graph_feats}.

\subsection{Line vessel graph L(G)}
\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figs/grph_des.png}
    \caption{Depiction of an exemplary vessel tree with the the spatial vessel Graph $\mathcal{G}(\mathcal{V},\mathcal{E})$ with nodes $(\mathcal{V})$ and edges $(\mathcal{E})$; additionally, a line graph  $L(\mathcal{G})$ of the spatial vessel graph $\mathcal{G}$ ; where each node (bifurcation point) becomes an edge; two nodes of $L(\mathcal{G})$ are adjacent if and only if their edges are incident in $\mathcal{G}$.}
    \label{fig:graphs}
\end{figure}
\label{Line_Graph}
As an alternative representation of whole brain vessel graphs, we convert our vessel graphs $\mathcal{G}$ to a corresponding line-graph representation, $L(\mathcal{G})$\cite{gross2018graph}. A line graph (depicted in Figure \ref{fig:graphs}) is a graph where the edges of the base graph $\mathcal{G}$ become nodes and an edge between the new nodes is created if and only if their edges are incident in $\mathcal{E}$. Edges are the most important aspects in our graph $\mathcal{E}$ because of their one-to-one correspondence to the vessels. Therefore, we wish to apply another set of graph-learning algorithms, namely node classification algorithms, to study their biological properties based on the rich set of vessel features. Hence, we construct an alternative representation with the help of line graph $L(\mathcal{G})$. We formally define $L(\mathcal{G}) := (\mathcal{V}',\mathcal{E}')$ where $\mathcal{V}'=\mathcal{E}$ and $\mathcal{E}'=\{\{e_{ij}, e_{ik}\}$ if $\exists \; (e_{ij}, e_{ik}) \in \mathcal{E}$\}.
\paragraph{Nodes:}
Now, the nodes in the line graph $\mathcal{V}'$ represent vessels or vessel segments, see Figure \ref{fig:graphs}. 
\paragraph{Node features:}
Thus, all edge features of $\mathcal{G}$ can now be used as node features for $L(\mathcal{G})$, see Table \ref{tab:graph_feats}. One of the key advantages of constructing the line graph is that we can now leverage a large number of prior techniques presented in node classification literature such as the use of vessel features in message passing.
\paragraph{Edges:}
Edges are defined as pairwise adjacencies of two nodes (vessels) \textit{if and only if} the corresponding edges in $\mathcal{G}$ are connected to a node $\mathcal{V}$. In practice, this means that nodes in $\mathcal{G}$ which are of degree $1$ disappear in $L(\mathcal{G})$ and that each node in $\mathcal{G}$ with a degree $\geq 2$ will create multiple edges in $L(\mathcal{G})$. 
\paragraph{Edge features:}
The spatial location given as node features in $\mathcal{G}$ can now be added as an edge feature.



==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/04_link_base.tex <==
\section{Benchmarking link prediction}
\label{Link_Base}
	

The formal goal of link prediction is to train a classifier $\mathcal{F}$ which predicts links in $\mathcal{E}_{\mbox{\textit{pred}}}$ as positive and negative labels, it can be formalized as follows $\mathcal{F} :\mathcal{E}_{\mbox{\textit{pred}}} \rightarrow \{0,1\}$.

From a biological perspective this task is relevant to correct missing and imperfect vessel graph connections, because the extracted graph may be over- or under-connected, due to artifacts and shortcoming of the segmentation and network extraction.

In order to provide initial baselines for vessel (link) prediction, we implemented 10 models. The following graph learning baselines were trained without edge features: the GCN by Kipf et al. \cite{kipf2016semi}, a GNN using the GraphSAGE operator \cite{hamilton2017inductive} and the SEAL GNN, a network aiming to learn general graph structure features from the local subgraph \cite{zhang2018link}. Furthermore, we trained a multilayer perceptron (MLP) on full batches based on Node2Vec features \cite{grover2016node2vec}. Apart from these, more traditional, heuristic-based methods were implemented for the task of link prediction, which include the Katz index \cite{katz1953new}, Common Neighbour, Page Rank and Adamic Adar \cite{adamic2003friends}, a measure which computes the closeness of nodes. These traditional methods make predictions based on the graph structure itself.



\subsection{Dataset curation - SEAL}	

\paragraph{Link sampling strategy:} 
\label{Link_Sampling}

The curation of a balanced training dataset requires the introduction of two types of edges. Similar to the SEAL paper \cite{zhang2018link}, we use the notion of \textit{positive edges} and \textit{negative edges}. Generally, positive edges are random samples of existing links and negative edges are samples of non-existent links between randomly chosen nodes of the dataset (which are included in the adjacency matrix). For positive edges, we utilize random samples of the existing edges of each graph. However, since our dataset includes 3D coordinates as the node features, their spatial nature makes selecting negative samples more challenging. A trivial random selection, which has been used in other state-of-the-art methods such as SEAL, would lead to biologically implausible edges, e.g. an edge between two nodes in different brain hemispheres. These can be easily distinguished based on the coordinates and thus would not provide useful information to the model. As such, models trained with trivial random sampling struggle with the link prediction task. To address this issue, we restrict negative edge sampling to a coordinate space which spatially surrounds the source node, and choose the target node by randomly selecting nodes that are located within the following cubic space around the source node: $\delta = \overline{l_{i,j}} + 2 \sigma $, where $\overline{l_{i,j}}$ denotes the average vessel length in $\mathcal{G}$. We note that this link sampling strategy is a first baseline and could be improved upon in future work.
\paragraph{Experiment:}
For our GCN based architectures we did an extensive grid-search of hyper-parameter combinations on a subset of the whole brain graph. We subsequently trained on the whole brain graphs. This intermediate step was necessary because exploring thousands of hyper-parameter combinations on the whole brain dataset is computationally infeasible. Implementation details and details on the hyperparameter search are indicated in supplementary Table \ref{tab:link_hyper_parameters}.
	
For the main experiment we sample all edges from one whole brain graph as positive edges $\mathcal{G(V,E)}$ (BALBc-1, Vessap, see Table \ref{tab:graph_numbers_nodes_edges})and randomly assign these to the training, validation and test set (80/10/10 split). Moreover, we sample an identical number of negative edges, i.e. non-existent but theoretically probable links according to the curation criterion described above. Next, we randomly shuffle all negative edges. Thus, we mitigate any bias in the negative train, validation and test splits and ensure a region-independent distribution. Subsequently, we randomly assign the negative edges to the train, validation and test set (80/10/10 split). This provides us with a balanced datast in regards to positive and negative edges.

We choose to only use the spatial node features for our experiment: ${x_n,y_n,z_n}$. This task is very hard because the algorithm essentially has to learn the vascular graph hierarchy purely on undirected relational and spatial information. 

\begin{table}[h!]
\footnotesize
\centering
\caption{\label{tab:results_link_pred} Results for the link prediction baselines.}
\begin{tabular}{| l||c|c|}
\hline
Algorithm  & \multicolumn{2}{|c|}{ROC AUC} \\
                        & validation & test  \\
\hline
Adamic Adar & 48.49  & 48.49   \\
Common Neighbors & 48.50  & 48.49  \\
Resource Allocation &48.49 & 48.50  \\
\hline
Matrix Factorization & 50.07   & 50.08  \\
MLP  &  57.98  &  58.02 \\
\hline
GCN GCN & 50.69  &  50.72  \\
GCN GCN + embeddings&  51.32 &  51.13  \\
GCN SAGE + embeddings   & 52.81  & 52.88 \\
GCN SAGE &  59.37 &  59.23  \\ % final
\hline
SEAL  &  \textbf{91.01} & \textbf{90.96} \\ % final
\hline
\end{tabular}
%}
\end{table}
Generally, traditional methods and simple GCN models performed poorly. Among the traditional methods tested, the MLP performed best. On the other hand, the SEAL implementation reached a superior performance and a strong inductive bias (ROC AUC $>90\%$). This improvement is in line with recent literature \cite{zhang2021revisiting}, which found a considerable performance improvement as a result of the employed labeling trick. This highlights that complex, dedicated graph-learning concepts need to be developed to address biologically inspired spatial graph challenges. A detailed experimental description and interpretation can be found in the Supplementary material, section \ref{Suppl_Link_Pred}. 



==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/05_node_base.tex <==
\section{Benchmarking vessel attribute classification}
\label{Node_Base}

Our formal goal of node classification is to train a classifier $\mathcal{F}$ which predicts a class label $\mathcal{Y}$ out of a set of possible classes $\mathcal{N}_n$ of a node $\mathcal{V}$, it can be formalized as follows $\mathcal{F} :\mathcal{V} \rightarrow \mathcal{Y}\in \mathcal{N}_n$.

Biologically, this task is relevant because the vessel radius is one of the most important parameters for blood flow; any task associated with flow modelling (such as stroke diagnosis and treatment) is heavily dependent on the diameter of the affected vessel. For example in stroke, a different treatment option is chosen based on the size of the vessel in the context of its local network topology. Therefore, reliably classifying vessel segments into categories such as arteries/veins, arterioles/venules and capillaries is relevant.  

For the secondary task of vessel radius (node) classification we implemented 7 graph and non-graph learning baselines discussed in the OGB paper \cite{hu2020open}. Among them node classification using an MLP initialized on N2Vec \cite{grover2016node2vec}, a simple GCN \cite{kipf2016semi}, a GNN using the GraphSAGE operator \cite{hamilton2017inductive}, the GraphSAINT algorithm which includes a mini-batch GCN\cite{zeng2019graphsaint}, the Scalable Inception Graph Neural Networks (SIGN)\cite{frasca2020sign} and the Cluster-GCN algorithm\cite{chiang2019cluster}.
Furthermore we implemented SpecMLP-W + C\&S and SpecMLP-W + C\&S + N2Vec, which use shallow models ignoring graph structure and standard label propagation techniques from semi-supervised learning methods \cite{huang2020combining}. 

\paragraph{Experiment:}
We split our three classes according to the minimum radius feature $\mu^{r}_{ij}$ into classes of $\mu^{r}_{ij}< 15\mu m;15-40\mu m$ and $>40\mu m$. Defined by the anatomy and properties of oxygen distribution these three classes are highly imbalanced. E.g. for the \textit{Vessap} datasets the distribution is roughly $95\%$, $4\%$ and $1\%$. Similarly to the link prediction task we carried out a grid search for optimal hyper-parameters, see Supplementary Table \ref{tab:node_hyper_parameters}. We randomly split the nodes into train, validation and test sets of (80/10/10) of one whole mouse brain (BALBc-1, Vessap, see Table \ref{tab:graph_numbers_nodes_edges}). We choose to use the following node features for our experiment: $l_{ij}$ , $d_{ij}$ and $\rho_{ij}$.

\begin{table}
\centering
\footnotesize
\caption{\label{tab:results_node_prediction} Results of the implemented node classification baselines. The performance scores are the weighted F1 score, one versus rest ROC AUC, class balanced accuracy and total accuracy (ACC).}

\begin{tabular}{| l||c|c|c|c|c|c |c|c |}
\hline
  & \multicolumn{2}{|c|}{F1 Score}  & \multicolumn{2}{|c|}{ROC AUC} &                                                 \multicolumn{2}{|c|}{Balanced ACC} & \multicolumn{2}{|c|}{ACC} \\
                        & valid & test & valid & test & valid & test & valid & test\\
\hline

GCN                                         & $75.74$   & $75.75$   
                                            & $67.23$   & $66.46$
                                            & $58.38$   & $56.83$
                                            & $62.94$   & $62.92$ \\
GraphSAGE                                   & $81.98$   & $81.98$   
                                            & $\mathbf{77.35}$ & $\mathbf{77.18}$
                                            & $\mathbf{71.82}$   & $\mathbf{71.33}$
                                            & $72.02$   & $71.98$ \\
GraphSAINT                                  & $77.46$   & $77.40$   
                                            & $71.38$   & $70.71$
                                            & $63.74$   & $62.51$
                                            & $64.88$   & $64.84$ \\
SIGN                                        & $74.46$   & $74.49$   
                                            & $67.26$   & $66.04$
                                            & $57.90$   & $55.88$
                                            & $61.25$   & $61.27$ \\
Cluster-GCN                                 & $\mathbf{86.10}$   & $\mathbf{86.06}$  
                                            & $\mathbf{77.91}$   & $\mathbf{77.43}$
                                            & $\mathbf{72.23}$   & $\mathbf{71.87}$
                                            & $\mathbf{77.47}$   & $\mathbf{77.41}$ \\
\hline
MLP                                         & $76.11$   & $76.11$   
                                            & $58.08$   & $57.79$
                                            & $42.36$   & $41.72$
                                            & $63.65$   & $63.61$ \\
SpecMLP-W + C\&S                        & $84.48$   & $84.55$   
                                            & $58.12$   & $58.54$
                                            & $42.20$   & $42.93$
                                            & $75.84$   & $75.91$ \\
SpecMLP-W +  + N2Vec             & $80.53$   & $80.63$   
                                            & $66.69$   & $66.20$
                                            & $59.04$   & $57.90$
                                            & $69.99$   & $70.10$ \\
\hline
\end{tabular}
\end{table}

For node classification, we find acceptable to high performance in our baselines 
by all the methods we tested. More complex graph models such as GraphSAGE and Cluster-GCN outperform simple GCNs on average over all metrics. According to the metrics which account for class imbalance i.e. ROC AUC and balanced ACC, graph neural networks outperform non-graph learning methods, for a detailed interpretation see Supplementary \ref{Suppl_Node_Class}. 



	


==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/06_Discussion.tex <==
\section{Discussion}
\label{Discussion}

In this work, we introduce and make publicly available a large dataset of vessel graphs representing the most comprehensive and highest resolution representation of the whole vascular connectome to-date. We provide this set of graphs as a new \say{baseline dataset} for machine learning on graphs and make it re-usable and easily accessible by leveraging widely employed open standards, such as the \textit{OGB} and \textit{PyTorch Geometric} dataloaders. 

To provide an example for the utilization of our dataset and to promote graph machine learning research in neuroscience, we provide two benchmarks: First, we benchmark vessel (link) prediction to improve the vascular connectome; second, we implement vessel (node) classification into three main anatomical categories on the line graph. We thus show that graph learning-based methods outperform traditional methods for vessel (node) classification. Moreover, we demonstrate that link prediction based solely on the spatial organization is a difficult task for most algorithms. However, we provide evidence that the combination of an appropriately chosen, complex GNN model (SEAL) with a labeling trick can achieve high accuracy on this task, paving the way for dedicated machine learning research on spatial (biological) graphs as a key to unlocking biological insight. 

\paragraph{Dataset bias:} While the dataset and the evaluation we provide are thorough, we note the following bias in our work: Our vascular graphs are constrained by the technical bias and limitations inherent to experimental imaging, such as artifacts in the clearing protocol and physical limitations concerning the resolution and isotropy of the microscopy. All specimen imaged in this study are males. Moreover, even state-of-the-art deep learning methods for segmentation presented in literature are only trained on incomplete sets of labeled data, leading to a model bias in segmentation. Further problems can occur from the known limitations of topological thinning-based methods for graph extraction \cite{drees2021scalable}. 

\paragraph{Limitations:} 

The sum of these effects and bias can impair the usefulness of our dataset for certain, highly specialised tasks, such as flow simulations using the Navier-Stokes equations, which are strongly dependent on accurate radius measurements. 

Moreover, benchmarking all available features, data and concepts was beyond the scope of our work. For instance, an extension to heterogeneous graph representations \cite{schlichtkrull2018modelingrgcn, vashishth2019composition}, the utilization of more features, the inclusion of more than one graph or of weighted graphs, where e.g. all edges (vessels) are weighted depending on an embedding of their radius, may facilitate an improved interpretation. 
In summary, we are convinced that both the machine learning concepts and the biological insight arising from our work can be translated to other tasks, such as graph extraction and refinement on different vascular or neuronal imaging techniques, artery and vein classification, and even vessel classification in inherently different medical imaging protocols such as angiography for stroke diagnosis. We are thus hopeful that our provision of high-quality data and strong baselines will stimulate future research in this area.


==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/11_datasheet.tex <==


%%%%%%%%%%%%%%% Datasheet for Datasets %%%%%%%%%%%%%%%%%%%%
\section{Datasheet for datasets}
This description is an additional documentation intended to enhance reproducibility and follows the \textbf{Datasheets for Datasets}\footnote{\url{https://arxiv.org/abs/1803.09010}} working paper developed for the machine learning community. 

\begin{itemize}

\item \textbf{For what purpose was the dataset created?}
To foster research development in machine learning for graphs, in particular its application to neuroscience - specifically the brain vessel graph composition.

\item \textbf{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}
The dataset was created thorough a collaborative effort by neuro-scientists and computer-scientists at the Technical University of Munich and the Helmholtz Zentrum München (under the supervision of Ali Ertuerk, Bjoern Menze and Stephan Günnemann).
  
\item \textbf{Who funded the creation of the dataset?} 
The creation of the dataset was funded only indirectly via the salaries of the scientists at the Technical University of Munich and the other corresponding affiliations of the authors. 

\end{itemize}

\subsection{Composition}

\begin{itemize}

\item \textbf{What do the instances that comprise the dataset represent?} 
Our dataset represents graph representations of the whole brain vasculature. We are providing two alternative representations of the vascular graph. First, a representation where individual vessels are represented as edges in a Graph; and second, the corresponding Line graph were vessels are represented as nodes. One can interpret the graph of a single mouse brain as a single instance. Alternatively one can interpret each vessel (edge) and bifurcation (node) as a physical instance. 

\item \textbf{How many instances are there in total (of each type, if appropriate)?}
By the instance definition of whole brain graphs as instances we are providing 17 graphs (with the option to generate the line graph) from 3 imaging sources as instances. In the future we plan to extend the dataset as soon as other whole brain vessel segmentations are made publicly available (open source).  

By the definition of vessels and bifurcation points we have millions of instances for each. Please see Table \ref{tab:graph_numbers_nodes_edges} for detailed numbers.


\item \textbf{Does the dataset contain all possible instances or is it a sample of instances from a larger set?} We are providing all available instances. 

\item \textbf{What data does each instance consist of?} In either case, please provide a description. By definition 1); each instance represents a whole mouse brains' vascular graph saved in the widely used CSV format. By definition 2) each node represents a bifurcation point and each edge a vessel. 

\item \textbf{Is there a label or target associated with each instance?} Yes, in case of the edge and node instances, the information from the extracted graphs (features) can be used as the instance labels. E.g. in our node classification benchmark we use the vessel radius binned in three classes as an instance label. 
  
\item \textbf{Is any information missing from individual instances?}
No, all of the information has been provided.

\item \textbf{Are relationships between individual instances made explicit?} 
In our dataset the instances (brain graphs) are independent.
  
\item \textbf{Are there recommended data splits (e.g., training, development/validation, testing)?} 
For the benchmark we split one whole brain into a train, validation and test set of 80/10/10.
  
\item \textbf{Are there any errors, sources of noise, or redundancies in the dataset?} Our graph extraction is based on experimental imaging and segmentation techniques. Therefore, errors and uncertainty are inherent. We discuss these in detail in our Limitations section in the conclusion. 

\item \textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?} The provided dataset is self-contained. 

\item \textbf{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals' non-public communications)?} No. 

\item \textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?} No. 

\item \textbf{Does the dataset relate to people?} No. 

\end{itemize}

\subsection{Collection process}

\begin{itemize}

\item \textbf{How was the data associated with each instance acquired?} The data was generated from a set of different publicly available datasets of whole murine brain images and segmentations. The specifics of the generation of each of these public segmentations are specified in the referenced literature and their licenses, see \ref{Individual_Licenses_Data}. 
    
\item \textbf{What mechanisms or procedures were used to collect the data?} We use the \textit{Voreen} framework \cite{drees2021scalable,meyer2009voreen} to generate graphs from segmentations. \textit{Voreen} is a software which runs on a CPU. 
    
\item \textbf{If the dataset is a sample from a larger set, what was the sampling strategy?} The dataset is complete. 

\item \textbf{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}
Only researchers (co-authors) of the Technical University of Munich and the Helmholtz Zentrum München were involved in the data collection process.

\item \textbf{Over what timeframe was the data collected?} Does this timeframe match the creation timeframe of the data associated with the instances (e.g., recent crawl of old news articles)?  The generation of the dataset, including dedicated research to gather the base segmentations and to optimize the graph extraction procedure took roughly one year. 

\item \textbf{Were any ethical review processes conducted (e.g., by an institutional review board)?} Our work is purely based on public and open sourced data. However, ethical review processes were carried out for each of these open sourced base segmentation sets:

The three graphs from Ji et al. \cite{ji2021brain} are based on animal experiments,  they followed the Guide for the Care and Use of Laboratory Animals and have been approved by the Institutional Animal Care and Use Committee, for details see \url{https://doi.org/10.1016/j.neuron.2021.02.006}.

The animal experiments for the nine datasets from the VesSAP paper \cite{todorov2020machine} were carried out under approval of the ethical review board of the government of Upper Bavaria (Regierung von Oberbayern, Munich, Germany), and in accordance with European directive 2010/63/EU for animal research, for details see \url{https://doi.org/10.1038/s41592-020-0792-1}. 

\item \textbf{Does the dataset relate to people?} No.

\end{itemize}

\subsection{Preprocessing/cleaning/labeling}

\begin{itemize}

\item \textbf{Was any preprocessing/cleaning/labeling of the data done ?} Yes, this actually constitutes a core contribution of our work, therefore please refer to Section \ref{Graph_Ext} in the main paper and to Supplementary section \ref{Suppl_Graph_Doc}.

\item \textbf{Was the 'raw' data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?} The raw data are the base segmentations. They are publicly available, the links are provided in Supplementary section \ref{Individual_Licenses_Data}.

\item \textbf{Is the software used to preprocess/clean/label the instances available?}
The \textit{Voreen} software used for the graph extraction is publicly available, see our github repo.
\end{itemize}

\subsection{Uses} 
\begin{itemize}
\item \textbf{Has the dataset been used for any tasks already?} In its current size and level of labeling detailization, the dataset was not used before (besides for the presented link prediction and node classification in this work). 

\item \textbf{Is there a repository that links to any or all papers or systems that use the dataset?} If so, please provide a link or other access point.
Yes, \url{https://github.com/jocpae/VesselGraph}.

\item \textbf{What (other) tasks could the dataset be used for?} In the main paper we discussed two standard tasks in machine learning on graphs; we think that our dataset can serve as a starting point for many interesting research directions in machine learning research and neurovascular research. 

\item \textbf{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?} No. 

\item \textbf{Are there tasks for which the dataset should not be used?} No. 
\end{itemize}

\subsection{Distribution}

\begin{itemize}

\item \textbf{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?} Our Dataset is open sourced under a CC Attribution-NonCommercial 4.0 International (CC BY-NC 4.0) License. Therefore all third parties can openly access it. 

\item \textbf{How will the dataset will be distributed (e.g., tarball  on website, API, GitHub)?} Yes, our DOI is \url{10.5281/zenodo.5301621}

\item \textbf{When will the dataset be distributed?} The dataset is available from the moment of submission. 

\item \textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?} Our Dataset is open sourced under a CC Attribution-NonCommercial 4.0 International (CC BY-NC 4.0) License.
\item \textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?} No. 
\item \textbf{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?} No.


\end{itemize}

\subsection{Maintenance}

\begin{itemize}

\item \textbf{Who is supporting/hosting/maintaining the dataset?}
The dataset is initially supported and maintained by the lead authors of this paper. The data is initially hosted on a university server and links are provided in the github repository \url{https://github.com/jocpae/VesselGraph}. In the long term we aim to incorporate our dataset into the open graph benchmark (OGB) initiative\footnote{\url{https://ogb.stanford.edu/}}. 

\item \textbf{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?} Of course via e-mail:  \url{johannes.paetzold@tum.de} and via the github repository, see question above. 

\item \textbf{Is there an erratum?} At this stage no, but we are happy to track them in a dedicated file in our github repository. 

\item \textbf{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?} Yes, we release the dataset on open platforms on which we plan to continuously update our dataset. Particularly to add novel whole brain vessel graphs to the dataset.
    
\item \textbf{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances?} The dataset does not relate to people. 
    
\item \textbf{Will older versions of the dataset continue to be supported/hosted/maintained?} When novel versions of the dataset will be released we will continue to host and maintain the old versions of the dataset.
    
\item \textbf{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?} We encourage other researches to exactly that. Depending on their contribution they can contribute to our github repository (in case of implementations) or reach out to us via e-mail in case they want to contribute graphs to the dataset. Our dataset and code are open sourced, see above. 

\end{itemize}


==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/21_table_hyper_link.tex <==
\begin{table}[h]
\centering
\tiny
\caption{\label{tab:link_hyper_parameters} Details of the hyper-parameters search for Link prediction with the selected parameters for the final training of each of our baseline models.}

\begin{tabular}{| l||l|l|l|}
\hline

Model                                    & Parameter Range & Selected Parameters & Model Select.\\
\hline
Matrix Factorization                 & lr $\in$ \{$1 \cdot10^{-3}, 1\cdot 10^{-4},
                                                1 \cdot10^{-5}$\}
                                                & lr = $1 \cdot10^{-5}$ &  epochs $3000$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $3$ &  \\
                                                & hidden channels  $\in$ \{$32,64,128,256$\}      
                                                & hidden channels = $64$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.2$ & \\

\hline 
MLP                                             & lr $\in$ \{$1 \cdot10^{-2},1 \cdot10^{-3},                                                    1\cdot 10^{-4}, 1 \cdot10^{-5}$\}
                                                & lr = $1 \cdot10^{-5}$ &  epochs $3000$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $4$  &  \\
                                                & hidden channels  $\in$ \{$128,256,512$\}      
                                                & hidden channels = $256$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.2$ & \\

\hline 
GCN    \cite{kipf2016semi}           & lr $\in$ \{$1 \cdot10^{-2},1 \cdot10^{-3}, 1\cdot 10^{-4},                                                      1\cdot 10^{-5}$\}
                                                & lr = $1 \cdot10^{5}$ &  epochs $3000$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $2$  &  \\
                                                & hidden channels  $\in$ \{$128,256,512$\}      
                                                & hidden channels = $256$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.2$ & \\
\hline 
GNN + N2Vec Embeddings \cite{grover2016node2vec}                                            &                                                  lr $\in$ \{$1 \cdot10^{-2},1 \cdot10^{-3}, 
                                                1\cdot 10^{-4}, 1\cdot 10^{-5}$\}
                                                & lr = $1 \cdot10^{-5}$ &  epochs $3000$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $2$  &  \\
                                                & hidden channels  $\in$ \{$128,256,512$\}      
                                                & hidden channels = $256$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.2$ & \\
\hline 
GNN + SAGE \cite{hamilton2017inductive}  
                                                & lr $\in$ \{$1 \cdot10^{-2},1 \cdot10^{-3},
                                                1\cdot 10^{-4},1\cdot 10^{-5}$\}
                                                & lr = $1 \cdot10^{-4}$ &  epochs $3000$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $3$  &  \\
                                                & hidden channels  $\in$ \{$128,256,512$\}      
                                                & hidden channels = $16$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.5$ & \\
                                                
                                                
\hline 
GNN + SAGE \cite{hamilton2017inductive}  + N2Vec  Embeddings \cite{grover2016node2vec}                                                  & lr $\in$ \{$1 \cdot10^{-02},1 \cdot10^{-3},
                                                1\cdot 10^{-4},1\cdot 10^{-5}$\} 
                                                & lr = $1 \cdot10^{-3}$ &  epochs $3000$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $2$  &  \\
                                                & hidden channels  $\in$ \{$128,256,512$\}      
                                                & hidden channels = $16$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.5$ & \\
% verified and checked!!!                                                
\hline 
SEAL \cite{zhang2018link}
                                                & lr $\in$ \{$1\cdot 10^{-4},1\cdot 10^{-5}$\}
                                                & lr = $ 1 \cdot10^{-4}$\} &  epochs $100$  \\
                                                & num of layers  $\in$ \{$2,3,4$\}          
                                                & num of layers  = $2$  &  \\
                                                & hidden channels  $\in$ \{$32,64,128$\}      
                                                & hidden channels = $32$ &  \\
                                                & dropout  $\in$ \{$0,0.2,0.5$\}
                                                & dropout = $0.0$ & \\
                                                & num of hops$\in$ \{$1,2,3$\}      
                                                & num of hops  = $1$ &  \\
                                                & labeling $\in$ \{drnl,de,de+,zo\}      
                                                & labeling = drnl & \\
                                                & model = {DGCNN, GCN}
                                                & model = {DGCNN} &\\
\hline
N2Vec \cite{grover2016node2vec}              & lr $\in$ \{$1\cdot10^{-2}, 1\cdot 10^{-3},
                                                              1 \cdot10^{-4},1 \cdot10^{-5},1 \cdot10^{-6}$\}
                                                & lr = $1 \cdot10^{-6}$\ &  epochs $2$  \\
                                                & walk length $\in$ \{$5,10,20$\}          
                                                & walk length = $5$  & \\
                                                & walks per\_node $\in$ \{$5,10,20$\}     
                                                & walks\_per\_node  = $10$ &  \\
                                                & embedding\_dim $\in$ \{$16,32,64,128,256$\}
                                                & embedding\_dim = $64$& \\
\hline                                                
\end{tabular}

\end{table}

==> Whole Brain Vessel Graphs A Dataset and Benchmark for Graph Learning and Neuroscience (VesselGraph)/21_table_hyper_node.tex <==
\begin{table}[h]
\centering
\caption{\label{tab:node_hyper_parameters} Details of the hyper-parameter search for node classification with the final parameters selected for the our baseline models.}
\tiny
\begin{tabular}{| l||l|l|l|}
\hline
Model                                         & Parameter Range & Selected Parameters & Model Select.\\
\hline 
Cluster-GCN                                     & lr $\in$ \{$2\cdot10^{-5}, 1\cdot10^{-4},
                                                      1\cdot10^{-3}, 3\cdot10^{-3}$\}           
                                                & lr = $3\cdot10^{-3}$
                                                & 1500 epochs   \\
                                                & number of layers $\in$ \{$3, 4, 5$\}                    
                                                & number of layers = $4$    
                                                &  \\
                                                & hidden channels $\in$ \{$128, 256, 512$\} 
                                                & hidden channels = $128$  
                                                &  \\
                                                & number of partitions $\in$ \{$3, 6, 9$\}  
                                                & number of partitions  = $9$ 
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.2, 0.5$\}  
                                                & dropout = 0.2 
                                                &  \\
\hline 
GNN                                             & lr $\in$ \{$2\cdot10^{-5}, 1\cdot10^{-4}, 1\cdot10^{-3},
                                                              3\cdot10^{-3}$\} 
                                                & lr = $3\cdot10^{-3} $ 
                                                & 1500 epochs   \\
                                                & number of layers $\in$ \{$3, 4, 5$\}                    
                                                & number of layers = $3$    
                                                &  \\
                                                & hidden channels $\in$ \{$32, 128, 256, 512, 1024$\} 
                                                & hidden channels = $256$ 
                                                &  \\
                                                & dropout $\in$ \{$0.1, 0.4, 0.5$\}  
                                                & dropout = $0.4 $
                                                &  \\
\hline 
GNN-SAGE                                        & lr $\in$ \{$2\cdot10^{-5}, 1\cdot10^{-4}, 1\cdot10^{-3},
                                                              3\cdot10^{-3}$\} 
                                                & lr = $3\cdot10^{-3}$  
                                                & $1500$ epochs   \\
                                                & number of layers $\in$ \{$2, 3, 4$\}                    
                                                & number of layers = $4$    
                                                &  \\
                                                & hidden channels $\in$ \{$32, 128, 256, 512, 1024$\}
                                                & hidden channels = $128 $
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.2, 0.4$\}  
                                                & dropout = $0.4$ 
                                                &  \\
\hline 
Graph-Saint                                     & lr $\in$ \{$1\cdot10^{-6}, 1\cdot10^{-5}, 1\cdot10^{-4}, 
                                                           1\cdot10^{-3}, 5\cdot10^{-3}, 1\cdot10^{-2}$\}
                                                & lr = $5\cdot10^{-4}  $
                                                & $1000$ epochs   \\
                                                & number of layers $\in$ \{$2, 3, 4$\}                    
                                                & number of layers = $4 $   
                                                &  \\
                                                & hidden channels $\in$ \{$64, 256, 512, 1024$\}                           
                                                & hidden channels = $64$ 
                                                &  \\
                                                & walk length $\in$ \{$3, 5, 7$\}   
                                                & walk length = $7$ 
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.35, 0.5$\}  
                                                & dropout = $0.35$
                                                &  \\
\hline 
SIGN                                            & lr $\in$ \{$1\cdot10^{-5}, 1\cdot10^{-4}, 1\cdot10^{-3},
                                                              5\cdot10^{-3}$\}
                                                & lr = $1\cdot10^{-3}$  
                                                & $1000$ epochs   \\
                                                & number of layers $\in$ \{$2, 3, 4$\}                    
                                                & number of layers = $3$    
                                                &  \\
                                                & hidden channels $\in$ \{$32, 64, 128, 256, 512, 1024$\}  
                                                & hidden channels = $128$ 
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.1, 0.3, 0.5$\}  
                                                & dropout = $0.1$
                                                &  \\

\hline 
MLP                                             & lr $\in$ \{$2\cdot10^{-5}, 1\cdot10^{-4}, 5\cdot10^{-4}, 
                                                           1\cdot10^{-3}, 3\cdot10^{-3}, 1\cdot10^{-2}$\}
                                                & lr = $1\cdot10^{-3} $ 
                                                & $1500$ epochs   \\
                                                & number of layers $\in$ \{$2, 3, 4$\}                    
                                                & number of layers = $3$   
                                                &  \\
                                                & hidden channels $\in$ \{$32, 128, 256, 512$\}
                                                & hidden channels = $256 $
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.3, 0.4$\}  
                                                & dropout = $0.0$
                                                &  \\
\hline 
SpecMLP-W + C\&S                                & lr $\in$ \{$1\cdot10^{-5}, 5\cdot10^{-4}, 1\cdot10^{-3}, 
                                                           3\cdot10^{-3}$\}
                                                & lr = $1\cdot10^{-3} $ 
                                                & $1500$ epochs   \\
                                                & number of layers $\in$ \{$3, 4, 5$\}                    
                                                & number of layers = $5$    
                                                &  \\
                                                & hidden channels $\in$ \{$128, 512, 1024$\}
                                                & hidden channels = $128 $
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.5$\}  
                                                & dropout = $0.5$
                                                &  \\
\hline
N2Vec                                           & lr $\in$ \{$1 \cdot10^{-5}, 1\cdot 10^{-3}, 
                                                              1 \cdot10^{-2}$\}
                                                & lr = $1 \cdot10^{-2}$\} 
                                                & $5$ epochs \\
                                                & walk length $\in$ \{$16, 40$\}           
                                                & walk length = $40$  
                                                &  \\
                                                & walks per node $\in$ \{$4, 10$\}      
                                                & walks per node  = $10$
                                                &  \\
                                                & embedding dim $\in$ \{$16,128$\}
                                                & embedding dim = $128$
                                                & \\
                                                & batch size $\in$ \{$16,128$\}
                                                & batch size = $128$
                                                & \\
                                                & epochs $\in$ \{$1, 5, 32$\}
                                                & epochs = $5$
                                                & \\
\hline
SpecMLP-W + C\&S + N2Vec                        & lr $\in$ \{$1\cdot10^{-5}, 5\cdot10^{-4}, 1\cdot10^{-3}, 
                                                           3\cdot10^{-3}$\}
                                                & lr = $1\cdot10^{-3} $ 
                                                & $1500$ epochs   \\
                                                & number of layers $\in$ \{$3, 4, 5$\}                    
                                                & number of layers = $5$    
                                                &  \\
                                                & hidden channels $\in$ \{$128, 512, 1024$\}
                                                & hidden channels = $128 $
                                                &  \\
                                                & dropout $\in$ \{$0.0, 0.5$\}  
                                                & dropout = $0.5$
                                                &  \\
\hline
\end{tabular}
\end{table}


